Exploring Content Selection in Summarization of Novel Chapters

We present a new summarization task, generating summaries of novel chapters using summary/chapter pairs from online study guides. This is a harder task than the news summarization task, given the chapter length as well as the extreme paraphrasing and generalization found in the summaries. We focus on extractive summarization, which requires the creation of a gold-standard set of extractive summaries. We present a new metric for aligning reference summary sentences with chapter sentences to create gold extracts and also experiment with different alignment methods. Our experiments demonstrate significant improvement over prior alignment approaches for our task as shown through automatic metrics and a crowd-sourced pyramid analysis. We make our data collection scripts available at https://github.com/manestay/novel-chapter-dataset .

==> savedtext.tex <==
o address this need, we are using data from  
online study guides such as CliffsNotes or NovelGuide to  develop an approach to generating summaries of novel chapters. The summaries of online study guides are quite abstractive, rarely using the exact language of the novel itself, many of which are from the 19th century . This presents a challenging scenario as the summaries use extensive paraphrasing when conveying the information from the novel (see the example summary and piece of the corresponding chapter for the novel {\em The Awakening}). Abstractive summarization methods are not currently sophisticated enough to generate such extensive revisions to extracted sentences, particularly when the quantity of available  summary/chapter pairs numbers in the tens of  thousands. 
